Fast Interpretable Greedy-Tree Sums

Modern machine learning has achieved impressive prediction performance, but often sacrifices interpretability, a critical consideration in high-stakes domains such as medicine. In such settings, practitioners often use highly interpretable decision tree models, but these suffer from inductive bias against additive structure. To overcome this bias, we propose Fast Interpretable Greedy-Tree Sums (FIGS), which generalizes the CART algorithm to simultaneously grow a flexible number of trees in summation. By combining logical rules with addition, FIGS is able to adapt to additive structure while remaining highly interpretable. Extensive experiments on real-world datasets show that FIGS achieves state-of-the-art prediction performance. To demonstrate the usefulness of FIGS in high-stakes domains, we adapt FIGS to learn clinical decision instruments (CDIs), which are tools for guiding clinical decision-making. Specifically, we introduce a variant of FIGS known as G-FIGS that accounts for the heterogeneity in medical data. G-FIGS derives CDIs that reflect domain knowledge and enjoy improved specificity (by up to 20% over CART) without sacrificing sensitivity or interpretability. To provide further insight into FIGS, we prove that FIGS learns components of additive models, a property we refer to as disentanglement. Further, we show (under oracle conditions) that unconstrained tree-sum models leverage disentanglement to generalize more efficiently than single decision tree models when fitted to additive regression functions. Finally, to avoid overfitting with an unconstrained number of splits, we develop Bagging-FIGS, an ensemble version of FIGS that borrows the variance reduction techniques of random forests. Bagging-FIGS enjoys competitive performance with random forests and XGBoost on real-world datasets.

==> figs/data_classification.tex <==
\begin{tabular}{lrr}
\toprule
                                         Name &  Samples &  Features \\
\midrule
% Ionosphere \cite{sigillito1989classification} &      351 &        34 \\
              Diabetes \cite{smith1988using} &      768 &         8 \\
                                German credit &     1000 &        20 \\
          Juvenile \cite{osofsky1997effects} &     3640 &       286 \\
                                  Recidivism &     6172 &        20 \\
             Credit \cite{yeh2009comparisons} &    30000 &        33 \\
                                  Readmission &   101763 &       150 \\
\bottomrule
\end{tabular}



% \begin{tabular}{lrr}
% \toprule
%                                          Name &  Samples &  Features \\
% \midrule
% % Ionosphere \cite{sigillito1989classification} &      351 &        34 \\
%               Diabetes \cite{smith1988using} &      768 &         8 \\
%                                 German credit &     1000 &        20 \\
%           Juvenile \cite{osofsky1997effects} &     3640 &       286 \\
%                                   Recidivism &     6172 &        20 \\
%              Credit \cite{yeh2009comparisons} &    30000 &        33 \\
%                                   Readmission &   101763 &       150 \\
% \bottomrule
% \end{tabular}

==> figs/data_classification_full.tex <==
\begin{tabular}{lrrrrr}
\toprule
                                         Name &  Samples &  Features &  Class 0 &  Class 1 &  Majority class \% \\
\midrule
% Ionosphere \cite{sigillito1989classification} &      351 &        34 &      126 &      225 &              64.1 \\
               Diabetes \cite{smith1988using} &      768 &         8 &      500 &      268 &              65.1 \\
                                German credit &     1000 &        20 &      300 &      700 &              70.0 \\
           Juvenile \cite{osofsky1997effects} &     3640 &       286 &     3153 &      487 &              86.6 \\
                                   Recidivism &     6172 &        20 &     3182 &     2990 &              51.6 \\
             Credit \cite{yeh2009comparisons} &    30000 &        33 &    23364 &     6636 &              77.9 \\
                                  Readmission &   101763 &       150 &    54861 &    46902 &              53.9 \\
\bottomrule
\end{tabular}

==> figs/data_regr.tex <==
\begin{tabular}{lrr}
\toprule
                                     Name &  Samples &  Features \\
\midrule
       Breast tumor \cite{romano2020pmlb} &   116640 &         9 \\
 California housing \cite{pace1997sparse} &    20640 &         8 \\
        Echo months \cite{romano2020pmlb} &    17496 &         9 \\
    Satellite image \cite{romano2020pmlb} &     6435 &        36 \\
        Abalone \cite{nash1994population} &     4177 &         8 \\
      Diabetes  \cite{efron2004least} &      442 &        10 \\
Friedman1 \cite{friedman1991multivariate} &      200 &        10 \\
Friedman2 \cite{friedman1991multivariate} &      200 &         4 \\
Friedman3 \cite{friedman1991multivariate} &      200 &         4 \\
\bottomrule
\end{tabular}

==> figs/data_regr_full.tex <==
\begin{tabular}{lrrrrrr}
\toprule
                                     Name &  Samples &  Features &  Mean &   Std &  Min &    Max \\
\midrule
       Breast tumor \cite{romano2020pmlb} &   116640 &         9 &  24.7 &  10.3 & -8.5 &   62.0 \\
 California housing \cite{pace1997sparse} &    20640 &         8 &   2.1 &   1.2 &  0.1 &    5.0 \\
        Echo months \cite{romano2020pmlb} &    17496 &         9 &  22.0 &  15.8 & -4.4 &   74.6 \\
    Satellite image \cite{romano2020pmlb} &     6435 &        36 &   3.7 &   2.2 &  1.0 &    7.0 \\
        Abalone \cite{nash1994population} &     4177 &         8 &   9.9 &   3.2 &  1.0 &   29.0 \\
      Diabetes  \cite{efron2004least} &      442 &        10 & 152.1 &  77.0 & 25.0 &  346.0 \\
Friedman1 \cite{friedman1991multivariate} &      200 &        10 &  14.7 &   5.2 &  2.5 &   26.5 \\
Friedman2 \cite{friedman1991multivariate} &      200 &         4 & 462.9 & 373.4 & 10.1 & 1657.0 \\
Friedman3 \cite{friedman1991multivariate} &      200 &         4 &   1.3 &   0.3 &  0.0 &    1.6 \\
\bottomrule
\end{tabular}

==> tables/prop_model_variables.tex <==
\begin{tabular}{lclclc}
\\
    \toprule
    \multicolumn{2}{c}{Traumatic Brain Injury} 
        & \multicolumn{2}{c}{Cervical Spine Injury} 
        & \multicolumn{2}{c}{Intra-Abdominal Injury}\\
     \cmidrule(lr){1-2}
     \cmidrule(lr){3-4}
     \cmidrule(lr){5-6}
     Variable & Coefficient & Variable & Coefficient & Variable & Coefficient\\
     \midrule
     No fontanelle bulging & 3.62 & Neck tenderness & 2.44 & Bike injury & 2.01 \\
     Amnesia & 2.07 & Neck pain & 2.18 & Abdomen pain & 1.66 \\
     Pedestrian stuck by vehicle  & 1.44 & Motor vehicle injury: other & 1.54 & Thoracic tenderness & 1.43 \\
     Headache & 1.39 & Hit by car & 1.47 & Hypotension & 1.23 \\
     Bike injury & 1.26 & Substantial injury: extremity & 1.35 & No abdomen pain & 0.98 \\
     \midrule
     Amnesia unknown & -1.31 & Midline tenderness unknown & -0.59 & Object struck abdomen & -0.46 \\
     Headache unknown & -1.53 & Neck tenderness unknown & -0.59 & MOI: unclear & -0.89 \\
     Fall down stairs & -1.57 & Not ambulatory & -0.66 & MOI: other & -1.20 \\
     Vomiting before injury & -1.78 & Predisposing condition & -0.97 & Abdomen pain unclear & -1.48 \\
     Fontanelle bulging unknown & -2.44 & Position: pre-ambulatory & -3.92 & Fall down stairs & -1.58 \\
    \bottomrule
\end{tabular}

==> tables/sim_results.tex <==
\begin{tabular}{lcccc}
    \toprule
    {} & ROC AUC & APS & Accuracy & F1 \\
    \midrule
    TAO & .376 (.07) & .498 (.04) & 59.0 (.02) & 58.0 (.04) \\
    TAO-SEP  & .475 (.04) & .573 (.03) & 58.3 (.02) & 60.4 (.03) \\
    CART & .370 (.07) & .495 (.04) & 56.5 (.02) & 54.7 (.03) \\
    CART-SEP & .475 (.04) & .573 (.03) & 58.3 (.02) & 60.4 (.03) \\
    FIGS & .470 (.04) & .539 (.04) & 58.5 (.02) & 55.5 (.03) \\
    FIGS-SEP & .475 (.04) & .573 (.03) & 58.3 (.02) & 60.4 (.03) \\
    \textbf{G-CART / \methodabbrv} & \textbf{.550} (.03) & \textbf{.644} (.03) & \textbf{65.8} (.03)  & \textbf{63.9} (.04) \\
    %\methodabbrv & \textbf{.550} (.03) & \textbf{.644} (.03) & \textbf{65.8} (.03) & \textbf{63.9} (.04) \\
    \bottomrule
\end{tabular}
